SelfAPR: Self-supervised Program Repair with Test Execution Diagnostics

Learning-based program repair has achieved good results in a recent series of papers. Yet, we observe that the related work fails to repair some bugs because of a lack of knowledge about 1) the application domain of the program being repaired, and 2) the fault type being repaired. In this paper, we solve both problems by changing the learning paradigm from supervised training to self-supervised training in an approach called SelfAPR. First, SelfAPR generates training samples on disk by perturbing a previous version of the program being repaired, enforcing the neural model to capture projectspecific knowledge. This is different from the previous work based on mined past commits. Second, SelfAPR executes all training samples and extracts and encodes test execution diagnostics into the input representation, steering the neural model to fix the kind of fault. This is different from the existing studies that only consider static source code as input. We implement SelfAPR and evaluate it in a systematic manner. We generate 1 039 873 training samples obtained by perturbing 17 open-source projects. We evaluate SelfAPR on 818 bugs from Defects4J, SelfAPR correctly repairs 110 of them, outperforming all the supervised learning repair approaches.

==> Listing/Closure_57.tex <==
\begin{listing}[t!]
\noindent\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 

<@\colorbox{red!60!}{-  if (target != null)  \{ }@>
<@\colorbox{green!50!}{+       if (target != null && target.getType() == Token.STRING)  \{ }@>   
       parent.detachFromParent();    
 }
\end{lstlisting}
\end{minipage}%
\caption{\approach correct patch generated for Closure-57 with the invocation requiresLevel.isOn() not exist in context }




\label{lst:closure-113}
\end{listing}

==> Listing/Jsoup-85.tex <==
\begin{listing}[t!]

\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 
         Validate.notNull(key);
<@\colorbox{red!60!}{-        this.key = key.trim();\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad }@>    
<@\colorbox{green!50!}{+        key = key.trim();\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad }@>    
Validate.notEmpty(key); // trimming could potentially make empty
<@\colorbox{green!50!}{+        this.key = key;\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \quad\quad\quad\quad  }@>    
         this.val = val;
\end{lstlisting}
\subcaption{The bug of Jsoup-85 and human-written patch}
\label{human-patch-jsoup-85}

\end{minipage}%
\hfill
\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 
         Validate.notNull(key);
         this.key = key.trim();
<@\colorbox{green!60!}{+ if (this.key!=null \&\&this.key.trim().length()==0)\{ \quad\quad\quad\quad }@> 
<@\colorbox{green!60!}{+ \quad\quad\quad\quad   throw  new IllegalArgumentException (" ") ; \quad\quad\quad\quad }@>   
<@\colorbox{green!60!}{ + \}\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad }@>   
 Validate.notEmpty(key);
\end{lstlisting}
\subcaption{\approach's patch}
\label{machine-patch-jsoup-85}
\end{minipage}%
\hfill


\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 
<@\colorbox{yellow!40!}{\textbf{Diagnostic: [FE] AssertionFailedError: Expected exception:} }@> 
<@\colorbox{yellow!40!}{\textbf{java.lang.IllegalArgumentException} \quad\quad\quad\quad\quad\quad\quad\quad\quad }@> 
    \end{lstlisting}
\subcaption{Diagnostics for Jsoup-85}
\label{jsoup-diagnostic}
\end{minipage}%
\caption{SUPREME's patch for Jsoup-85 guided by diagnostics}
\label{listing-jsoup-85}
\end{listing}

==> Listing/codeInsert.tex <==
\begin{listing}[t!]

\begin{lstlisting} [firstnumber=419] 
<@{\textbf{\underline{$Rule_{9}$:} replacement by a donor statement}}@>
    - target statement
    + donor statement 
<@{\textbf{\underline{$Rule_{10}$:} transplant a donor statement }}@>
    +  donor statement;
       target statement;
    -  donor statement; // randomness to be removed
<@{\textbf{\underline{$Rule_{11}$:} wrap target statement with a donor condition: if, else, else if}}@>
    + if (exp1) {
         statement1;....
    +}
<@{\textbf{\underline{$Rule_{12}$:} insert a donor block (if, loop, etc)}}@>
    + if(exp1) {
    +   statement1;....
    + }  
\end{lstlisting} 
\caption{Perturbation  based on code transplantation.}
 \label{listinginsert}
\end{listing}



==> Listing/codeRemoval.tex <==
\begin{listing}[t!]

\begin{lstlisting} [firstnumber=419] 
<@{\textbf{\underline{$Rule_{13}$:} removal of single statement}}@>
      if (exp1!=null && exp1>exp2) {
    -    statement 1; 
         statement 2;
     }           
<@{\textbf{\underline{$Rule_{14}$:} removal of if condition (unwrap block)}}@>
    - if (exp1!=null && exp1>exp2) {
         statement1; statement2;
    - }           
<@{\textbf{\underline{$Rule_{15}$:} removal of AST block}}@>
    - for (exp1) {
    -     statement; ....
    -     return exp;
    - }          
          


\end{lstlisting} 
\caption{Perturbation based on code removal.}
\label{listing-removal}
\end{listing}





% \begin{listing}[t!]
% \noindent\begin{minipage}[b]{0.5\textwidth}
%     \begin{lstlisting} [firstnumber=419] 
%   Partial  - if (exp1!=null && exp1>exp2) {
%           + if (exp1!=null) {
%     \end{lstlisting}
 
%      \subcaption{Partial line removal}
%   \label{motivate-human-patch}  
%     \end{minipage}%
%     \hfill
%     \begin{minipage}[b]{0.49\textwidth}
%     \begin{lstlisting}[firstnumber=419] 
%     if (exp1!=null && exp1>exp2) {
%   -  statement; ....
%     }
   
%     \end{lstlisting}
 
%     \subcaption{Single line removal}
%  \label{motivate-noncompile-patch}   
% \end{minipage}%
% \hfill
%     \begin{minipage}[b]{0.49\textwidth}
%     \begin{lstlisting}[firstnumber=419] 
%   - if (exp1!=null && exp1>exp2) {
%   -         statement; ....
%   - }

%     \end{lstlisting} 
%     \subcaption{Continuous line block removal}
%     \label{motivate-correct-patch} 
% \end{minipage}%
% \hfill
%     \begin{minipage}[b]{0.49\textwidth}
%     \begin{lstlisting}[firstnumber=419] 
%   - if (exp1!=null && exp1>exp2) {
%           statement; ....
%   - }
%     \end{lstlisting} 
%     \subcaption{Noncontinuous line block removal}
%     \label{motivate-correct-patch} 
% \end{minipage}%
% \label{lst:coderemoval}
% \end{listing}

==> Listing/jsoup-41.tex <==
\begin{listing}[t!]
\noindent\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 
<@\colorbox{red!60!}{-        return this == o; }@>     
<@\colorbox{green!50!}{+ return tag.equals(element.tag); }@> //human-written patch
<@\colorbox{green!50!}{+  return tag!= null \&\& tag.equals (element.tag) ;}@> //SUPREME patch at Top-2.

 

 
 
 
 
\end{lstlisting}
\end{minipage}%
\caption{improves the human-patch}
\label{lst:jsoup-41}
\end{listing}

==> Listing/lang-21.tex <==
\begin{listing}[t!]
\noindent\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 


return 
(cal1.get(Calendar.MILLISECOND)==cal2.get(Calendar.MILLISECOND)&&
cal1.get(Calendar.SECOND) == cal2.get(Calendar.SECOND) &&
cal1.get(Calendar.MINUTE) == cal2.get(Calendar.MINUTE) &&
<@\colorbox{red!60!}{-  cal1.get(Calendar.HOUR)  ==  cal2.get(Calendar.HOUR) \&\& \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad }@>   
<@\colorbox{green!50!}{+ cal1.get(Calendar.HOUR\_OF\_DAY)  ==  cal2.get(Calendar.HOUR\_OF\_DAY)  \&\& \quad\quad\quad }@> 
cal1.get(Calendar.DAY_OF_YEAR) == cal2.get(Calendar.DAY_OF_YEAR)&&
cal1.get(Calendar.YEAR) == cal2.get(Calendar.YEAR) &&
cal1.get(Calendar.ERA) == cal2.get(Calendar.ERA) &&
cal1.getClass() == cal2.getClass());
 
\end{lstlisting}
\subcaption{Bug Lang-21 and human-written patch}
\end{minipage}%
\hfill
\noindent\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 

//SUPREME patch adds a stronger comparison on Calendar.MONTH
<@\colorbox{green!50!}{+ cal1.get(Calendar.HOUR\_OF\_DAY)  ==  cal2.get(Calendar.HOUR\_OF\_DAY)  \&\& \quad\quad\quad}@> 
<@\colorbox{green!50!}{+  cal1.get(Calendar.MONTH)  ==  cal2.get(Calendar.MONTH) \&\& \quad\quad\quad\quad\quad\quad\quad\quad\quad}@> 
\end{lstlisting}
\subcaption{\approach's patch for  Lang-21}
\label{patch-lang21}
\end{minipage}%

\caption{\approach's patch for Lang-21 not exists in the content context and project-specific knowledge to improve the human-patch.}
\label{lst-lang-21}
\end{listing}

==> Listing/lang-8.tex <==
\begin{listing}[t!]

\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] 

 public void appendTo(StringBuffer buffer, Calendar calendar) {            
<@\colorbox{green!50!}{+    TimeZone zone = calendar.getTimeZone();  }@>          
if (zone.useDaylightTime()  && calendar.get(Calendar.DST_OFFSET) != 0) {     buffer.append(getTimeZoneDisplay(zone, true, mStyle, mLocale));






\end{lstlisting}



\caption{Two bugs repaired by SUPREME with tokens outside the buggy context but learned from project-specific training samples }


\label{lst:closure-domain}
\end{listing}

==> Listing/lang21-single.tex <==
\begin{listing}[t!]
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white},basicstyle=\footnotesize\ttfamily,]


    
<@\colorbox{red!40!}{- cal1.get(Calendar.HOUR) == cal2.get(Calendar.HOUR)\quad\quad\quad\quad\quad\quad}@>
<@\colorbox{green!40!}{+ cal1.get(Calendar.HOUR\_OF\_DAY)==cal2.get(Calendar.HOUR\_OF\_DAY)}@>




\end{lstlisting}
\caption{The \approach's patch for Lang-21, identical to human-developers. }
\label{lst-lang-21}


\end{listing}

==> Listing/listing-cli-34.tex <==
\begin{listing}[t!]
\noindent\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white}] //
Cli_34_Option
@@ -71,3 +71,3 @@
     /** the type of this Option */
-    private Class type;
+    private Class type = String.class;

// Cli_34_OptionBuilder.java
@@ -83,3 +83,3 @@
         longopt = null;
-        type = null;
+        type = String.class;
         required = false;
         
\end{lstlisting}
\end{minipage}%
\caption{\approach correct patch generated for Cli-34}
\label{lst:cli-34}
\end{listing}

==> Listing/listing-mockito-34.tex <==
\begin{listing}[t!]

\begin{minipage}[b]{0.49\textwidth}

\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white},basicstyle=\scriptsize\ttfamily] 

for (Matcher m : matchers) {            
<@\colorbox{red!40!}{- if (m instanceof CapturesArguments) \{ \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad  \quad\quad\quad\quad }@>        
<@\colorbox{green!40!}{+ if (m instanceof CapturesArguments \&\& i.getArguments().length>k)\{   }@>  ((CapturesArguments) m).captureFrom(i.getArguments()[k]);            
  }
\end{lstlisting}



\subcaption{\approach's patch for Mockito-34, identical to the human-written patch. }
\end{minipage}%
\hfill
\begin{minipage}[b]{0.49\textwidth}
\begin{lstlisting} [firstnumber=419,backgroundcolor=\color{white},basicstyle=\scriptsize\ttfamily] 
<@\colorbox{yellow!40!}{Diagnostic: [FE] ArrayIndexOutOfBoundsException \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad}@> 
    \end{lstlisting}
\subcaption{Diagnostic for bug Mockito-34.}
\end{minipage}%
\caption{Patch for Mockito-34 guided by diagnostics, only repaired by \approach.}
\label{listing-mockito-34}
\end{listing}

==> Table/different.tex <==
\begin{table}[t!]
\small
\renewcommand{\arraystretch}{1.4}
 \begin{tabular}{p{0.35\linewidth} p{0.15\linewidth} p{0.15\linewidth} p{0.18\linewidth}}
\hline
Mode & Accuracy \\
\hline
SynFix & around(74.89\%) \\
Our work & 71.4\%\\
\hline
\end{tabular}
\caption{Repair accuracy on 10000 random Blackbox testing set}	
\label{tab:blackbox}
\end{table}

%ls -1 | wc -l

==> Table/novelty_table.tex <==
\begin{table}[t!]
\scriptsize
\renewcommand{\arraystretch}{1.2}
 \begin{tabular}{p{0.35\linewidth}cccccc}
\hline
Neural repair model &self-supervised & multi-task  & test-case specification \\
\hline
SequenceR(TSE'19)  \cite{SEQUENCER} & \xmark & \xmark & \xmark  \\
CoCoNUT (ISSTA'20) \cite{CoCoNuT} & \xmark  & \xmark & \xmark\\
CURE (ICSE'21) \cite{CURE-icse21} & \xmark & \xmark & \xmark \\
Recoder(FSE'21) \cite{Recoder} & \xmark  & \xmark & \xmark\\
MODIT(ASE'21) \cite{modit-ase21} & \xmark & \xmark  & \xmark\\
RewardRepair(ICSE'22)  \cite{RewardRepair-icse22}&  \xmark  &  \xmark  & \cmark \\


DrRepair(ICML'20)\cite{BIFI-ICML21} & \cmark &  \xmark  &  \xmark \\
BIFI(ICML'21)\cite{BIFI-ICML21} & \cmark &  \xmark  &  \xmark \\
\hline
our work  & \cmark  &\cmark&\cmark\\

\hline
\end{tabular}
\caption{Comparison with existing neural program repair models}	
\label{tab:dataset}
\end{table}

==> Table/testcase.tex <==
\begin{table}[t!]
\small
\renewcommand{\arraystretch}{1}
 \begin{tabular}{p{0.35\linewidth}lll}
\hline
NullPointerException &&\\
AssertionFailedError && \\
IndexOutOfBoundsException && \\
ArrayIndexOutOfBoundsException && \\
IllegalArgumentException && \\
ComparisonFailure&&\\
CustomizedException && \\
StackOverflowError && \\
RuntimeException &&\\
IllegalStateException \\
could be multiple\\
ComparisonFailure relates to condition!!!  \\
\hline
\end{tabular}
\caption{}	
\label{tab:blackbox}
\end{table}

%ls -1 | wc -l
